Vehicular Safety Applications and Approaches: A Technical Survey

This paper proposes an extensive overview of safety applications and approaches as it relates to automated driving from the prospectives of sensor configurations, vehicle dynamics modelling, tyre modeling, and estimation approaches. First, different Advanced-Driver Assistance Systems (ADAS) are introduced along with the main sensing components and technologies. Then, different kinematics modelling of vehicles and tyres are discussed. Finally, various communicational technologies and architectures along with self-driving modules are presented. Moreover, some interesting perspectives for future research are listed based on the extensive experience of the authors. The objective of this study is to teach and guide the beginner and expert for choosing the most suitable approach for autonomous driving applications in safety and stability targeted issues.

==> introduction.tex <==
\section{Introduction}
%stats in norway and weather-related crashes
%analysis for beginners and experts
%recent failures of SD and the auto industry
%Company Data, Morgan Stanley Research US cost savings from accidents.
